Mining Best Closed Itemsets for Projection-antimonotonic Constraints in Polynomial Time

The exponential explosion of the set of patterns is one of the main challenges in pattern mining. This challenge is approached by introducing a constraint for pattern selection. One of the first constraints proposed in pattern mining is support (frequency) of a pattern in a dataset. Frequency is an anti-monotonic function, i.e., given an infrequent pattern, all its superpatterns are not frequent. However, many other constraints for pattern selection are neither monotonic nor anti-monotonic, which makes it difficult to generate patterns satisfying these constraints. In order to deal with nonmonotonic constraints we introduce the notion of "projection antimonotonicity" and SOFIA algorithm that allow generating best patterns for a class of nonmonotonic constraints. Cosine interest, robustness, stability of closed itemsets, and the associated delta-measure are among these constraints. SOFIA starts from light descriptions of transactions in dataset (a small set of items in the case of itemset description) and then iteratively adds more information to these descriptions (more items with indication of tidsets they describe).

==> makefile <==
MAIN_FILE = icde16-Sofia-bin
MAIN_FILE_COMPILE=$(MAIN_FILE).tex
PRECOMPIELD_NAME=precompiled
PRECOMPIELD_DEP=$(shell ./find-deps.bash "tex/static.tex")
TIKZFLD = ./tikz/

RMFILESLIST = *.mtc* *.aux *.bak *.bbl *.bcf *.blg *.log *.out *.toc *.tdo _region.* *.run.xml *.flg *.idx *.maf _region_.* *~ *.ilg *.ind  *.fls *.fdb_latexmk *.M* *.gz *.fmt \#* *.nav *.snm precompiled.pdf
RMFILESCMD = $(patsubst %,-iname "%" -o,$(RMFILESLIST)) -false

TIME     = /usr/bin/time -p
LATEXMK  = latexmk -halt-on-error -pdf -pdflatex="pdflatex -fmt $(PRECOMPIELD_NAME) --synctex=1 -interaction=nonstopmode" # -shell-escape" 
FMTPDFLATEX=pdftex -ini -jobname="$(PRECOMPIELD_NAME)" -interaction=nonstopmode "&pdflatex" mylatexformat.ltx 

PDFLATEX = pdflatex -interaction=nonstopmode -output-directory 
PDFCROP  = pdfcrop
RM       = /bin/rm -f

StandAloneGraphicsTeXFiles = $(wildcard $(TIKZFLD)/*.tex)

PDFGraphics = $(patsubst %.tex,%.pdf,$(StandAloneGraphicsTeXFiles))

#LatexFiles = $(shell find . -path $(TIKZFLD) -prune -o -type f -iname '*.tex')
LatexFiles = $(shell ./find-deps.bash "$(MAIN_FILE).tex")

CurrentInclude = $(shell ./find-include.bash "$(MAIN_FILE).tex" "" $(CurrentFile))
CurrentIncludeGUARDSuffix = \#INCLUDE\#
CurrentIncludeGUARD = $(patsubst %,%$(CurrentIncludeGUARDSuffix),$(CurrentInclude))

#Includes = $(shell ./extract-includes.bash '\input{$(MAIN_FILE)}')
#IncludesPDF = $(patsubst %.tex,%.pdf,$(Includes))
#IncludesAUX = $(patsubst %.tex,%.aux,$(Includes))

COMPILE = $(TIME) $(LATEXMK) -jobname=$(MAIN_FILE) $(MAIN_FILE_COMPILE)
COMPILE_ALL = $(COMPILE) 

#----------------------init done--------------------------------

default : $(MAIN_FILE).pdf

# No difference for fast and standard in the case of small documents
#fast : $(CurrentIncludeGUARD)
fast : $(MAIN_FILE).pdf

# Forcing to recompile every time, latexmk will make a check
.PHONY : FORCE_MAKE
$(MAIN_FILE).pdf : $(MAIN_FILE).bcf $(PRECOMPIELD_NAME).fmt $(MAIN_FILE).tex $(LatexFiles) $(PDFGraphics) FORCE_MAKE
	/home/leshyk/PhD/GitDB/scripts-linux/correct-library-mendeley.bash
	/home/leshyk/PhD/GitDB/scripts-linux/clear-library.sh
	$(COMPILE_ALL)

$(MAIN_FILE).bcf : FORCE_MAKE
	test ! -f $(MAIN_FILE).bcf || grep '</bcf:controlfile>' $(MAIN_FILE).bcf || ( echo 'BCF file is corrupted, removing...' && rm $(MAIN_FILE).bcf )

$(PRECOMPIELD_NAME).fmt : $(PRECOMPIELD_DEP)
	touch $(PRECOMPIELD_NAME).mtc0
	$(FMTPDFLATEX)  $(MAIN_FILE_COMPILE)

$(TIKZFLD)%.pdf : $(TIKZFLD)%.tex
	$(PDFLATEX) $(TIKZFLD) $< 

clean : .PHONY
	@find $(RMFILESCMD) | xargs -I{} rm -r '{}'

depclean : clean
	$(RM) $(TIKZFLD)*.pdf
	#$(RM) $(IncludesPDF)

distclean : depclean
	$(RM) $(MAIN_FILE).pdf

noop : .PHONY
	@echo 'noop DONE'
#------------------------------------------------------
# for fast compiling of one include
.SECONDEXPANSION:

$(CurrentIncludeGUARD) : %$(CurrentIncludeGUARDSuffix) : $$(shell ./find-deps.bash %.tex) $(PRECOMPIELD_NAME).fmt $(MAIN_FILE).tex $(PDFGraphics) FORCE_MAKE
	@sed -i 's+\\begin{document}+\\includeonly{$(patsubst %$(CurrentIncludeGUARDSuffix),%,$@)}\\begin{document}+' $(MAIN_FILE_COMPILE)
	$(COMPILE) && echo "Compiled" >> $@

#--------------------------------------------------------
# For fast compiling of chapters. Syncinc will not work.

#incr: $(IncludesPDF) 
	#pdftk $(IncludesPDF) cat output $(MAIN_FILE).pdf

#.SECONDEXPANSION:

#$(IncludesPDF): %.pdf: %.tex $$(shell ./find-deps.bash %.tex) $(MAIN_FILE).tex $(PRECOMPIELD_NAME).fmt  $(PDFGraphics) 
## Checking if all aux exists. If not should recompile all.
#$(CHECK_AUX_COMPILE_ALL)
#cp $(MAIN_FILE).tex $(MAIN_FILE_COMPILE)
#sed -i 's+\\begin{document}+\\includeonly{$(patsubst %.pdf,%,$@)}\\begin{document}+' $(MAIN_FILE_COMPILE)
#$(TIME) $(LATEXMK) '-jobname=$(MAIN_FILE)' $(MAIN_FILE_COMPILE)
#cp $(MAIN_FILE).pdf $@



==> tex/tbl-krimp.tex <==
\begin{table}[t]
	\centering
	\resizebox{0.8\columnwidth}{!}{
	\begin{tabular}{l|c|c|c|c}
	\hline\hline
	Dataset & \# Cand. & Type & Time & Size \\
	\hline
	\multirow{2}{*}{Mushrooms}
	& 96235 & $\Sigma$ & 22 & 275937 \\
	& 105430 & Cls & 2.2 & 277992 \\

	& 9469 & $\Sigma$ & 2.8 & 354916 \\
	& 10006 & Cls & 0.2 & 494640 \\

	& 718 & $\Sigma$ & 0.4 & 519945 \\
	& 728 & Cls & 0.1 & 752711 \\
	\hline
	\multirow{2}{*}{Chess}
	& 98528 & $\Sigma$ & 19 & 295401 \\
	& 99629 & Cls & 1 & 375214 \\
	& 9639 & $\Sigma$ & 2.1 & 320360 \\
	& 9970 & Cls & $<$0.1 & 459190 \\
	& 928 & $\Sigma$ & 0.3 & 373205 \\
	& 999 & Cls & $<$0.1 & 532128 \\
	\hline
	\multirow{2}{*}{Plants}
	& 94130 & $\Sigma$ & 174 & 732309 \\
	& 96819 & Cls & 7.5 & 901354 \\
	& 9602 & $\Sigma$ & 22 & 793977 \\
	& 9923 & Cls & 3.4 & 1011407 \\
	& 1000 & $\Sigma$ & 3 & 954132 \\
	& 1006 & Cls & 0.9 & 1151570 \\
	\hline\hline
	\end{tabular}
	}
	\caption{Compression with KRIMP based on \textDelta-stable itemsets and closed itemsets.}
	\label{tbl:krimp}
\end{table}


==> tex/tbl-measures-behaviour.tex <==
\begin{table*}
	\centering
	\resizebox{\textwidth}{!}{
	\begin{tabular}{l||ccc|ccc|ccc||ccc|ccc|ccc||ccc|ccc|ccc}
		\hline\hline
		\multirow{2}{*}{Datasets} & \multicolumn{9}{c||}{Decreasing order} & \multicolumn{9}{c||}{Increasing order} & \multicolumn{9}{c}{Random order}\\
		\cline{2-28}
		& \multicolumn{3}{c|}{$L=10^3$} & \multicolumn{3}{c|}{$L=10^4$} & \multicolumn{3}{c||}{$L=10^5$}
		& \multicolumn{3}{c|}{$L=10^3$} & \multicolumn{3}{c|}{$L=10^4$} & \multicolumn{3}{c||}{$L=10^5$}
		& \multicolumn{3}{c|}{$L=10^3$} & \multicolumn{3}{c|}{$L=10^4$} & \multicolumn{3}{c}{$L=10^5$}
		\\
		\cline{2-28}
		& $t$ & \# & $\theta$ & $t$ & \# & $\theta$ & $t$ & \# & $\theta$ 
		& $t$ & \# & $\theta$ & $t$ & \# & $\theta$ & $t$ & \# & $\theta$ 
		& $t$ & \# & $\theta$ & $t$ & \# & $\theta$ & $t$ & \# & $\theta$ 
		\\
		\hline
		Mushrooms 
		&$<1$&0.99&181
		&2&0.87&49
		&39&0.89&7

		&1&0.99&181
		&6&0.87&49
		&38&0.89&7

		&$<1$&0.99&181
		&3&0.87&49
		&117&0.89&7	 
		\\

		Chess 
		&$<1$&0.997&97
		&2&0.92&69
		&17&0.94&46	 
		
		&1&0.88&144
		&4&0.24&84
		&38&0.68&49
		
		&$<1$&0.65&103
		&2&0.92&69
		&19&0.94&46	 
		\\

		Plants
		&1&1&147
		&14&0.96&70	 
		&146&0.94&37

		&3&1&147
		&29&0.96&70
		&263&0.94&37	 

		&1&1&147
		&14&0.96&70
		&143&0.94&37
		\\

		Cars 
		&$<1$&0.94&19
		&$<1$&0.61&0
		&$<1$&0.06&0 

		&$<1$&0.86&22
		&$<1$&0.61&0
		&$<1$&0.06&0 

		&$<1$&0.94&19
		&$<1$&0.6&0
		&$<1$&0.06&0 
		\\
		%Cars 
		%&&&
		%&&&
		%&&&

		%&&&
		%&&&
		%&&&

		%&&&
		%&&&
		%&&&	 
		\hline\hline
	\end{tabular}
	}
	\caption{Evaluation results of \AlgoName{} algorithm for \textDelta-measure.}
	\label{tbl:measures-behaviour}
\end{table*}

